Efficient Adaptation of Deep Neural Networks for Semantic Segmentation in Space Applications

In recent years, the application of Deep Learning techniques has shown remarkable success in various computer vision tasks, paving the way for their deployment in extraterrestrial exploration. Transfer learning has emerged as a powerful strategy for addressing the scarcity of labeled data in these novel environments. This paper represents one of the first efforts in evaluating the feasibility of employing adapters toward efficient transfer learning for rock segmentation in extraterrestrial landscapes, mainly focusing on lunar and martian terrains. Our work suggests that the use of adapters, strategically integrated into a pre-trained backbone model, can be successful in reducing both bandwidth and memory requirements for the target extraterrestrial device. In this study, we considered two memory-saving strategies: layer fusion (to reduce to zero the inference overhead) and an ``adapter ranking'' (to also reduce the transmission cost). Finally, we evaluate these results in terms of task performance, memory, and computation on embedded devices, evidencing trade-offs that open the road to more research in the field.

==> suppl_classic_alg.tex <==
\subsection{Performance of Traditional Methods: \textit{Canny} and \textit{Otsu} Algorithms}

While this work focuses on Deep Learning (DL) techniques and their optimization, we also evaluated traditional algorithms on the same dataset to provide a fair comparison. As outlined by Thompson and Casta\~no~\cite{thompson2007performance}, traditional methods rely mainly on edge detection and thresholding for image segmentation. However, additional operations, such as contour classification, are required to assign detected regions to specific classes (e.g., distinguishing sky from terrain or rocks using criteria like contour size or threshold values).\\
The primary advantage of these algorithms is their applicability to any dataset without requiring training, eliminating the need for large datasets and the computational cost of training, which are significant for ML/DL approaches. Considering also the purpose of this work, this inherent adaptability makes them robust to domain changes, with performance depending solely on data quality and intrinsic characteristics and providing quick and automatic flexibility..\\
Despite these strengths, traditional methods generally underperform compared to DL models. For instance, as shown in Table \ref{tab:classic_alg} and noted by Thompson and Casta\~no~\cite{thompson2007performance}, traditional methods achieve an accuracy of around 60\% for rock segmentation in space imagery, compared to over 90\% achieved by DL approaches (Table \ref{tab:encoders}).

In this work, we implemented two well-known different algorithms on our three-classes datasets: the Canny edge detector \cite{canny_alg} and the Otsu thresholding \cite{otsu_alg}. Both of them are the base of the traditional computer vision approach: the former evaluates the gradient of the image, searching for steep changes, while the latter provides autonomous thresholding based on the image variance. Furthermore, we exploit their strengths by building a hybrid method, combining them. In the hybrid approach, \textit{Otsu} masks the background (sky and terrain), and \textit{Canny} refines rock detection. Note that these methods require grayscale images for processing. Results on the \textit{SMo} dataset are summarized in Table \ref{tab:classic_alg}, with visual examples in Fig. 
\ref{fig:classic_alg_comparison}. For consistency, the same train-validation-test split was used for DL methods.


\begin{table*}[h]
\centering
\begin{tabular}{ccccccc}
\multirow{3}{*}{\textbf{Algorithm}} & \multicolumn{2}{c}{\multirow{2}{*}{\textbf{Accuracy [\%]}}} & \multicolumn{2}{c}{\textbf{Balanced}} & \multicolumn{2}{c}{\multirow{2}{*}{\bf IoU [\%]}}\\
 & & & \multicolumn{2}{c}{\textbf{Accuracy [\%]}} & &    \\
 & \textit{SMo} & \textit{Marsdataset}  & \textit{SMo} & \textit{Marsdataset}  & \textit{SMo} & \textit{Marsdataset} \\
\toprule
\textit{Otsu}   & 86.15 & 67.19 & 66.73 & 48.50 & 59.10 & 27.08 \\
\textit{Canny}  & 49.20 & 42.38 & 38.74 & 37.55 & 28.74 & 15.03 \\
\textit{Hybrid} & 56.20 & 44.36 & 67.59 & 45.98 & 45.74 & 20.01 \\
\bottomrule
\end{tabular}
\caption{Performance of traditional algorithms (\textit{Canny}, \textit{Otsu}, and \textit{Hybrid}) on the \textit{SMo} dataset.}
\label{tab:classic_alg}
\end{table*}


\begin{figure*}[h]
    \centering
    \includegraphics[width = 0.8\textwidth]{figures/gt_300.pdf}
    \caption{Comparison of traditional methods (\textit{Canny}, \textit{Otsu}, and \textit{Hybrid}) with DL results on the \textit{SMo} dataset.}
    \label{fig:classic_alg_comparison}
\end{figure*}

As observed in Table \ref{tab:classic_alg} and Fig.~\ref{fig:classic_alg_comparison}, traditional methods struggle with rock segmentation. While \textit{Otsu} effectively identifies terrain and sky (high accuracy), it often detects only rock shadows (lower balanced accuracy). On the other hand, \textit{Canny} identifies better the rocks' edges but fails to capture the shapes accurately.  Due to these issues, we built \textit{Hybrid} that provides a good compromise between the two, improving rock detection but still achieving only $67.6\%$ accuracy compared to $\sim96\%$ for u-Nets.

Results on the Martian dataset further highlight the limitations of traditional methods. In this case, the different physical environments play a main role: the Moon's high contrast (dark sky and grayscale landscape) supports better the segmentation of these techniques. On the other hand, Mars' atmospheric effects, such as dust storms and sunlight scattering, reduce the contrast between sky and terrain, making more difficult the edges and background distinctions and leading to èsignificantly worse performance.\\

For these reasons, we discard the traditional approach for rock segmentation and especially for the domain adaptation task. Besides its great advantages, its poor performances overall and on the Martian landscapes make the DL techniques more preferable and potentially more promising.
